Slope-Dependent Rendering of Parallel Coordinates to Reduce Density Distortion and Ghost Clusters

Parallel coordinates are a popular technique to visualize multi-dimensional data. However, they face a significant problem influencing the perception and interpretation of patterns. The distance between two parallel lines differs based on their slope. Vertical lines are rendered longer and closer to each other than horizontal lines. This problem is inherent in the technique and has two main consequences: (1) clusters which have a steep slope between two axes are visually more prominent than horizontal clusters. (2) Noise and clutter can be perceived as clusters, as a few parallel vertical lines visually emerge as a ghost cluster. Our paper makes two contributions: First, we formalize the problem and show its impact. Second, we present a novel technique to reduce the effects by rendering the polylines of the parallel coordinates based on their slope: horizontal lines are rendered with the default width, lines with a steep slope with a thinner line. Our technique avoids density distortions of clusters, can be computed in linear time, and can be added on top of most parallel coordinate variations. To demonstrate the usefulness, we show examples and compare them to the classical rendering.

==> chapters/7-figures-old.tex <==
\begin{figure*}
    \centering
    \begin{tabular}{ cccc } 
        \includegraphics[width=.24\linewidth]{pictures/bias-1.png} &
        \includegraphics[width=.24\linewidth]{pictures/bias0.png} &
        \includegraphics[width=.24\linewidth]{pictures/bias1.png} &
        \includegraphics[width=.24\linewidth]{pictures/bias2.png} \\
        (a) $P=-1$ & (b) Regular ($P=0$) & (c) Adjusted ($P=1$) & (d) Over-Adjusted ($P=2$)
    \end{tabular}
    \caption{\textbf{Distortion in synthetic data with equally distributed random noise.} An unbiased view on the same-sized clusters is only provided by our adjustment method (3), while usual renderings exhibit a significant over-emphasis on diagonal clusters (2), which is exaggerated in (1). The same over-emphasis as put on diagonal clusters in (2) is put on horizontal clusters instead in (4).}
    \label{fig:bias}
\end{figure*}

%===================================================================================

\begin{figure*}
  \label{fig:ghost}
  \begin{centering}
    \begin{tabular}{ cccc } 
      %(a) 
      %&
      %\includegraphics[width=.19\linewidth]{n-1.png}
      %&
      \includegraphics[width=.24\linewidth,height=.14\linewidth]{n0.png} &
      \includegraphics[width=.24\linewidth,height=.14\linewidth]{n1.png} &
      \includegraphics[width=.24\linewidth,height=.14\linewidth]{n2.png} &
      \includegraphics[width=.24\linewidth,height=.14\linewidth]{n5.png} \\
      (a) $P=0$ & (b) $P=1$ & (c)  $P=2$ & (d) $P=5$
    \end{tabular}
  \end{centering}
  \caption{Effect of parameter $P$ on pattern visualization in uniformly distributed random noise. (a) shows the usual rendering method with occurring fake patterns. The distorting effects are effectively countered with our adjustment technique in (b). Over-adjusting arguably further improves the visualization in cases such as (c). Detrimental effects of over-adjusting are visible and in (d).
  }
\end{figure*}

